Nonasymptotic one-and two-sample tests in high dimension with unknown covariance structure

Let $\mathbf{X} = (X_i)_{1\leq i \leq n}$ be an i.i.d. sample of square-integrable variables in $\mathbb{R}^d$, \GB{with common expectation $\mu$ and covariance matrix $\Sigma$, both unknown.} We consider the problem of testing if $\mu$ is $\eta$-close to zero, i.e. $\|\mu\| \leq \eta $ against $\|\mu\| \geq (\eta + \delta)$; we also tackle the more general two-sample mean closeness (also known as {\em relevant difference}) testing problem. The aim of this paper is to obtain nonasymptotic upper and lower bounds on the minimal separation distance $\delta$ such that we can control both the Type I and Type II errors at a given level. The main technical tools are concentration inequalities, first for a suitable estimator of $\|\mu\|^2$ used a test statistic, and secondly for estimating the operator and Frobenius norms of $\Sigma$ coming into the quantiles of said test statistic. These properties are obtained for Gaussian and bounded distributions. A particular attention is given to the dependence in the pseudo-dimension $d_*$ of the distribution, defined as $d_* := \|\Sigma\|_2^2/\|\Sigma\|_\infty^2$. In particular, for $\eta=0$, the minimum separation distance is ${\Theta}( d_*^{\frac{1}{4}}\sqrt{\|\Sigma\|_\infty/n})$, in contrast with the minimax estimation distance for $\mu$, which is ${\Theta}(d_e^{\frac{1}{2}}\sqrt{\|\Sigma\|_\infty/n})$ (where $d_e:=\|\Sigma\|_1/\|\Sigma\|_\infty$). This generalizes a phenomenon spelled out in particular by Baraud (2002).

==> macrogilles_main_modif_sp.tex <==
%Packages standard

%\RequirePackage[latin1]{inputenc}





\RequirePackage{comment}
\RequirePackage{graphicx}
\RequirePackage{amsmath,amsfonts}
\RequirePackage{color}
\RequirePackage{bm}
\RequirePackage{stmaryrd}


%Theoremes

% \ifx \skiptheorems \thiscommandisnotdefinedtralala  
%                  %teste si \skiptheorems est non-defini

% %\RequirePackage{amsthm}

% \ifx \gillesfrench \thiscommandisnotdefinedtralala  

% \spnewtheorem{theorem}{Theorem}[section]
% \spnewtheorem{proposition}[theorem]{Proposition}
% \spnewtheorem{corollary}[theorem]{Corollary}
% \spnewtheorem{lemma}[theorem]{Lemma}


% \theoremstyle{definition}
% \spnewtheorem{definition}[theorem]{Definition}
% \spnewtheorem{property}[theorem]{Property}
% \spnewtheorem{example}[theorem]{Example}

% \theoremstyle{remark}
% \spnewtheorem{remark}[theorem]{Remark}

% \else

% \newtheorem{theorem}{Théorème}[section]
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{corollary}[theorem]{Corollaire}
% \newtheorem{lemma}[theorem]{Lemme}


% \theoremstyle{definition}
% \newtheorem{definition}[theorem]{Définition}
% \newtheorem{property}[theorem]{Propriété}
% \newtheorem{example}[theorem]{Example}


% \theoremstyle{remark}
% \newtheorem{remark}[theorem]{Remarque}

% \fi
% \fi

% Fontes

\newcommand{\mtc}{\mathcal}
\newcommand{\mbf}{\bm}

% Some black magick to remove annoying extra spaces before/after \left* and \right*

\let\originalleft\left
\let\originalright\right
\renewcommand{\left}{\mathopen{}\mathclose\bgroup\originalleft}
\renewcommand{\right}{\aftergroup\egroup\originalright}


% Accents tildes over/underline etc

\newcommand{\wt}[1]{{\widetilde{#1}}}
\newcommand{\wh}[1]{{\widehat{#1}}}
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\ul}[1]{\underline{#1}}

% Delimiteurs divers

\RequirePackage{xstring}




\newcommand{\paren}[2][a]{%
\IfEqCase{#1}{%
{a}{\left(#2\right)}%
{0}{(#2)}%
{1}{\big(#2\big)}%
{2}{\Big(#2\Big)}%
{3}{\bigg(#2\bigg)}%
{4}{\Bigg(#2\Bigg)}%
}[\PackageError{paren}{Undefined option to paren: #1}{}]%
}
\newcommand{\norm}[2][a]{%
\IfEqCase{#1}{%
{a}{\left\lVert#2\right\rVert}%
{0}{\lVert#2\rVert}%
{1}{\big\lVert#2\big\rVert}%
{2}{\Big\lVert#2\Big\rVert}%
{3}{\bigg\lVert#2\bigg\rVert}%
{4}{\Bigg\lVert#2\Bigg\rVert}%
}[\PackageError{norm}{Undefined option to norm: #1}{}]%
}
\newcommand{\brac}[2][a]{%
\IfEqCase{#1}{%
{a}{\left[#2\right]}%
{0}{[#2]}%
{1}{\big[#2\big]}%
{2}{\Big[#2\Big]}%
{3}{\bigg[#2\bigg]}%
{4}{\Bigg[#2\Bigg]}%
}[\PackageError{brac}{Undefined option to brac: #1}{}]%
}
\newcommand{\inner}[2][a]{%
\IfEqCase{#1}{%
{a}{\left\langle#2\right\rangle}%
{0}{\langle#2\rangle}%
{1}{\big\langle#2\big\rangle}%
{2}{\Big\langle#2\Big\rangle}%
{3}{\bigg\langle#2\bigg\rangle}%
{4}{\Bigg\langle#2\Bigg\rangle}%
}[\PackageError{inner}{Undefined option to inner: #1}{}]%
}
\newcommand{\abs}[2][a]{
\IfEqCase{#1}{%
{a}{\left\vert#2\right\rvert}%
{0}{\vert#2\rvert}%
{1}{\big\vert#2\big\rvert}%
{2}{\Big\vert#2\Big\rvert}%
{3}{\bigg\vert#2\bigg\rvert}%
{4}{\Bigg\vert#2\Bigg\rvert}%
}[\PackageError{abs}{Undefined option to abs: #1}{}]%
}

\newcommand{\set}[2][a]{
\IfEqCase{#1}{%
{a}{\left\{#2\right\}}%
{0}{\{#2\}}%
{1}{\big\{#2\big\}}%
{2}{\Big\{#2\Big\}}%
{3}{\bigg\{#2\bigg\}}%
{4}{\Bigg\{#2\Bigg\}}%
}[\PackageError{set}{Undefined option to set: #1}{}]%
}

\newcommand{\ind}[2][a]{{\mbf{1}\set[#1]{#2}}}

% Autres

\newcommand{\np}{_{_-}}
\newcommand{\pp}{_{_+}}
\newcommand{\defeq}{\stackrel{\cdot}{=}} % this is for
                                % definition-equal, not for number 2
                                % [This comment is (c) Gabór L. ]
\newcommand{\bydef}{:=}       % an alternative to defeq

\newcommand{\intr}[1]{\llbracket #1 \rrbracket}

% Operateurs proba

\newcommand{\var}[2][a]{{\rm Var}\brac[#1]{#2}}
\newcommand{\cov}[2][a]{{\rm Cov}\brac[#1]{#2}} 
\newcommand{\e}[2][a]{\mbe\brac[#1]{#2}}
\newcommand{\ee}[3][a]{\mbe_{#2}\brac[#1]{#3}}
\newcommand{\prob}[2][a]{\mbp\brac[#1]{#2}}
\newcommand{\probb}[3][a]{\mbp_{#2}\brac[#1]{#3}}


% Operateurs

\def\argmin{\mathop{\rm Arg\,Min}}
\def\argmax{\mathop{\rm Arg\,Max}}
\def\sgn{\mathop{\rm Sgn}}
\def\tr{\mathop{\rm Tr}}


% abbrev lettres grecques

\newcommand{\al}{\alpha}
\newcommand{\om}{\omega}
\newcommand{\eps}{\varepsilon}

% abbrev lettres mathcal

\def\cA{{\mtc{A}}}
\def\cB{{\mtc{B}}}
\def\cC{{\mtc{C}}}
\def\cD{{\mtc{D}}}
\def\cE{{\mtc{E}}}
\def\cF{{\mtc{F}}}
\def\cG{{\mtc{G}}}
\def\cH{{\mtc{H}}}
\def\cI{{\mtc{I}}}
\def\cK{{\mtc{K}}}
\def\cL{{\mtc{L}}}
\def\cM{{\mtc{M}}}
\def\cN{{\mtc{N}}}
\def\cO{{\mtc{O}}}
\def\cP{{\mtc{P}}}
\def\cQ{{\mtc{Q}}}
\def\cR{{\mtc{R}}}
\def\cS{{\mtc{S}}}
\def\cT{{\mtc{T}}}
\def\cU{{\mtc{U}}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}

% abbrev lettres mathbb

\newcommand{\mbe}{\mathbb{E}}
\newcommand{\mbr}{\mathbb{R}}
\newcommand{\mbc}{\mathbb{C}}
\newcommand{\mbp}{\mathbb{P}}
\newcommand{\mbq}{\mathbb{Q}}
\newcommand{\mbi}{\mathbb{I}}
\newcommand{\mbn}{\mathbb{N}}
\newcommand{\mbz}{\mathbb{Z}}
\newcommand{\mbs}{\mathbb{S}}
\newcommand{\mbx}{\mathbb{X}}


% abbrev lettres en gras

\newcommand{\bA}{{\bm{A}}}
\newcommand{\bB}{{\bm{B}}}
\newcommand{\bC}{{\bm{C}}}
\newcommand{\bD}{{\bm{D}}}
\newcommand{\bE}{{\bm{E}}}
\newcommand{\bF}{{\bm{F}}}
\newcommand{\bG}{{\bm{G}}}
\newcommand{\bH}{{\bm{G}}}
\newcommand{\bI}{{\bm{I}}}
\newcommand{\bU}{{\bm{U}}}
\newcommand{\bV}{{\bm{V}}}
\newcommand{\bW}{{\bm{W}}}
\newcommand{\bX}{{\bm{X}}}
\newcommand{\bY}{{\bm{Y}}}
\newcommand{\bZ}{{\bm{Z}}}


\newcommand{\bp}{{\bm{p}}}
\newcommand{\boldf}{{\bm{f}}}
\newcommand{\bs}{{\bm{s}}}
\newcommand{\bx}{{\bm{x}}}
\newcommand{\by}{{\bm{y}}}
\newcommand{\bz}{{\bm{z}}}
\newcommand{\bw}{{\bm{w}}}
\newcommand{\bv}{{\bm{v}}}
\newcommand{\ba}{{\bm{a}}}
\newcommand{\bb}{{\bm{b}}}
\newcommand{\bt}{{\bm{t}}}
\newcommand{\bj}{{\bm{j}}}
% frak

\newcommand{\fP}{{\mathfrak{P}}}
\newcommand{\fK}{{\mathfrak{K}}}


%
% \newcommand{\red}[1]{\textcolor{red}{#1}}
%



% % TODO command

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %% A command to put notes in a draft

% \newcounter{nbdrafts}
% \setcounter{nbdrafts}{0}
% \makeatletter
% \newcommand{\checknbdrafts}{
% \ifnum \thenbdrafts > 0
% \@latex@warning@no@line{**********************************************************************}
% \@latex@warning@no@line{* The document contains \thenbdrafts \space draft note(s)}
% \@latex@warning@no@line{**********************************************************************}
% \fi}
% \newcommand{\todo}[1]{\addtocounter{nbdrafts}{1}{\color{red} #1}}
% \makeatother

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

